Extraction of hierarchical functional connectivity components in human brain using resting-state fMRI

The study of hierarchy in networks of the human brain has been of significant interest among the researchers as numerous studies have pointed out towards a functional hierarchical organization of the human brain. This paper provides a novel method for the extraction of hierarchical connectivity components in the human brain using resting-state fMRI. The method builds upon prior work of Sparse Connectivity Patterns (SCPs) by introducing a hierarchy of sparse overlapping patterns. The components are estimated by deep factorization of correlation matrices generated from fMRI. The goal of the paper is to extract interpretable hierarchical patterns using correlation matrices where a low rank decomposition is formed by a linear combination of a high rank decomposition. We formulate the decomposition as a non-convex optimization problem and solve it using gradient descent algorithms with adaptive step size. We also provide a method for the warm start of the gradient descent using singular value decomposition. We demonstrate the effectiveness of the developed method on two different real-world datasets by showing that multi-scale hierarchical SCPs are reproducible between sub-samples and are more reproducible as compared to single scale patterns. We also compare our method with existing hierarchical community detection approaches. Our method also provides novel insight into the functional organization of the human brain.

==> extra_files/HSCP_map.tex <==
\begin{figure*}[h!tbp]
\begin{subfigure}{0.48\textwidth}
    \centering
\begin{minipage}[ct]{\textwidth}
\centering
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [A{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.22]{extra_files/brain/complete1.png}},styleA
    [2{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain/2.png}},styleA]
    [8{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain/8.png}},styleA]    
     ]
  ]
\end{forest}
\caption{Component A comprises of 2 and 8}
\end{minipage}
\end{subfigure}
\vspace{1em}
\hfill
\begin{subfigure}{0.48\textwidth}
\begin{minipage}[ct]{\textwidth}
\centering
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [B{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.22]{extra_files/brain/complete2.png}},styleA
    [1{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain/1.png}},styleA]
    [3{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain/3.png}},styleA]
     [6{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain/6.png}},styleA
        ]
     ]
  ]
\end{forest}
\caption{Component B comprises of 1,3 and 6}
\end{minipage}
\end{subfigure}
\vspace{1em}
\begin{subfigure}{0.63\textwidth}
    \centering
\begin{minipage}[ct]{\textwidth}
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [C{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.2]{extra_files/brain/complete3.png}},styleA
    [4{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain/4.png}},styleA]
    [5{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain/5.png}},styleA]
    [8{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain/8.png}},styleA] 
    [9{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain/9.png}},styleA]  
     ]
  ]
\end{forest}
\caption{Component C comprises of 4, 5, 8 and 9}
\end{minipage}
\end{subfigure}
\begin{subfigure}{0.37\textwidth}
    \centering
\begin{minipage}[ct]{\textwidth}
\centering
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [D{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.2]{extra_files/brain/complete4.png}},styleA
    [7{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain/7.png}},styleA]
    [10{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain/10.png}},styleA]
     ]
  ]
\end{forest}
\caption{Component D comprises of 7 and 10}
\end{minipage}
\end{subfigure}
   \caption{Hierarchical components derived from HCP dataset showing the connection between 10 fine scale components ($\mathbf{W}_1$) denoted from 1 to 10 and 4 coarse scale components ($\mathbf{W}_1\mathbf{W}_2$) denoted from A to D. Nodes with red and blue color are correlated among themselves, but are anitcorrelated with each other. Note that blue color does not need to be necessarily associate with positive or negative correlation because the colors can be flipped without affecting the solution. 8 fine scale components ($\mathbf{W}_1$). 2 and 8 show different regions of Default Mode anti-correlated with the Salience and Cingulo-Opercular system. 5 show different regions of default mode anti-correlated with the sensori-motor areas. 3 and 6 shows different regions of Visual system anti-correlated with Salience and Default Mode.}
    \label{fig:comp}
\end{figure*}

==> extra_files/HSCP_map2.tex <==
\begin{figure*}[h!tbp]
\begin{subfigure}{0.48\textwidth}
    \centering
\begin{minipage}[ct]{\textwidth}
\centering
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [A{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.22]{extra_files/brain2/complete1.png}},styleA
    [4{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/4.png}},styleA]
    [9{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/9.png}},styleA]
     [10{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/10.png}},styleA
        ]
     ]
  ]
\end{forest}
\caption{Component A comprises of 4, 9 and 10}
\end{minipage}
\end{subfigure}
\vspace{1em}
\hfill
\begin{subfigure}{0.48\textwidth}
\begin{minipage}[ct]{\textwidth}
\centering
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [B{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.22]{extra_files/brain2/complete2.png}},styleA
    [2{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/2.png}},styleA]
    [6{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/6.png}},styleA]
     [7{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/7.png}},styleA
        ]
     ]
  ]
\end{forest}
\caption{Component B comprises of 2, 6 and 7}
\end{minipage}
\end{subfigure}
\vspace{1em}
\begin{subfigure}{0.63\textwidth}
    \centering
\begin{minipage}[ct]{\textwidth}
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [C{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.22]{extra_files/brain2/complete3.png}},styleA
    [1{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/1.png}},styleA]
    [5{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/5.png}},styleA]
     [9{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.24]{extra_files/brain2/9.png}},styleA
        ]
     ]
  ]
\end{forest}
\caption{Component C comprises of 1, 5 and 9}
\end{minipage}
\end{subfigure}
\begin{subfigure}{0.37\textwidth}
    \centering
\begin{minipage}[ct]{\textwidth}
\centering
\begin{forest}
  styleA/.style={top color=white, bottom color=white},
  styleB/.style={%
    top color=white,
    bottom color=red!20,
    delay={%
      content/.wrap value={##1\\{\includegraphics[scale=.5]{hand}}}
    }
  },
  for tree={
    rounded corners,
    draw,
    align=center,
    top color=white,
    bottom color=blue!20,
  },
  forked edges,
  [D{ \includegraphics[trim={1cm 3cm 1cm 2cm},clip,scale=0.2]{extra_files/brain2/complete4.png}},styleA
    [1{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain2/1.png}},styleA]
    [8{ \includegraphics[trim={3cm 1.1cm 3cm 1cm},clip,scale=0.22]{extra_files/brain2/8.png}},styleA]
     ]
  ]
\end{forest}
\caption{Component D comprises of 1 and 8}
\end{minipage}
\end{subfigure}
   \caption{Hierarchy}
    \label{fig:comp}
\end{figure*}

==> extra_files/hetero.tex <==
\begin{figure*}[h!tbp]
    \begin{subfigure}[b]{\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
                %\includegraphics[trim={0cm 0.1cm 4cm 0.1cm},clip,trim={0cm 0.1cm 3cm 0.1cm},clip,width=\textwidth,height=20em]{extra_files/Hetero/cluster2.png}
        \includegraphics[width=0.9\textwidth,height=6cm]{extra_files/1_1.png}
    
    %\end{minipage}
    %\begin{minipage}[t]{0.49\textwidth}
     %   \centering
      %          \includegraphics[trim={0cm 0.1cm 4cm 0.1cm},clip,trim={0cm 0.1cm 3cm 0.1cm},clip,width=\textwidth]{extra_files/Hetero/cluster1.png}

    
    %\end{minipage}
    \end{subfigure}
    \centering
        \begin{subfigure}[b]{0.65\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{extra_files/Hetero/level1.png}
    
 
    \end{subfigure}
    \caption{Heterogeneity captured by fine scale components in HCP. The color indicates the strength ($\mathbf{\Lambda}_1$) of each component present in a subject. Respective components are displayed below each component id. Maximum strength of a component across subjects  is fixed to be 1 for comparison purpose.}
    \label{fig:hetero}
    \end{figure*}

==> extra_files/hetero1.tex <==
\begin{figure}
        \centering

    \begin{subfigure}[b]{0.48\textwidth}
        \centering
    \includegraphics[width=\textwidth]{extra_files/1_2.png}

    \end{subfigure}
    \centering
        \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part1_1.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part2_1.png}
    \end{subfigure}
     \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part3_1.png}
    \end{subfigure}
     \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part4_1.png}
    \end{subfigure}
    
     \centering
        \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part1_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part2_2.png}
    \end{subfigure}
     \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part3_2.png}
    \end{subfigure}
     \begin{subfigure}[b]{0.08\textwidth}
       %\begin{minipage}[t]{0.49\textwidth}
        \centering
      \includegraphics[width=0.6\textwidth]{extra_files/brain1/part4_2.png}
    \end{subfigure}
    
    
    \caption{Heterogeneity captured by coarse scale components in HCP. The color indicates the strength ($\mathbf{\Lambda}_2$) of each component present in a subject. Respective components are displayed below each component id. Maximum strength of a component across subjects  is fixed to be 1 for comparison purpose.}
    \label{fig:hetero1}
\end{figure}

==> extra_files/hetero2.tex <==
    \begin{figure}
    \begin{minipage}[t]{.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{extra_files/cluster1.png}
        \subcaption{Heterogeneity captured by subjects of cluster 1}
    \end{minipage}
    \begin{minipage}[t]{.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{extra_files/cluster2.png}
        \subcaption{Heterogeneity captured by subjects of cluster 2}
    \end{minipage}

        \caption{Heterogeneity captured by fine scale components in HCP. The color indicates the strength ($\mathbf{\Lambda}_1$) of each component present in a subject. Maximum strength of a component across subjects  is fixed to be 1 for comparison purpose.}
    \label{fig:hetero}
\end{figure}
